Learning to Predict Trustworthiness with Steep Slope Loss

Understanding the trustworthiness of a prediction yielded by a classifier is critical for the safe and effective use of AI models. Prior efforts have been proven to be reliable on small-scale datasets. In this work, we study the problem of predicting trustworthiness on real-world large-scale datasets, where the task is more challenging due to high-dimensional features, diverse visual concepts, and large-scale samples. In such a setting, we observe that the trustworthiness predictors trained with prior-art loss functions, i.e., the cross entropy loss, focal loss, and true class probability confidence loss, are prone to view both correct predictions and incorrect predictions to be trustworthy. The reasons are two-fold. Firstly, correct predictions are generally dominant over incorrect predictions. Secondly, due to the data complexity, it is challenging to differentiate the incorrect predictions from the correct ones on real-world large-scale datasets. To improve the generalizability of trustworthiness predictors, we propose a novel steep slope loss to separate the features w.r.t. correct predictions from the ones w.r.t. incorrect predictions by two slide-like curves that oppose each other. The proposed loss is evaluated with two representative deep learning models, i.e., Vision Transformer and ResNet, as trustworthiness predictors. We conduct comprehensive experiments and analyses on ImageNet, which show that the proposed loss effectively improves the generalizability of trustworthiness predictors. The code and pre-trained trustworthiness predictors for reproducibility are available at https://github.com/luoyan407/predict_trustworthiness.

==> depd/fig_anal_featinput.tex <==
\begin{figure}[!t]
	\centering
	\subfloat{\includegraphics[width=0.32\textwidth]{fig/analysis/anal_featinput_ce}    } \hfill
	\subfloat{\includegraphics[width=0.32\textwidth]{fig/analysis/anal_featinput_focal}    } \hfill
	\subfloat{\includegraphics[width=0.32\textwidth]{fig/analysis/anal_featinput_ss}    } \\
	\caption{\label{fig:anal_featinput}
    	Analysis of taking the features of the classifier as input to the oracle on the ImageNet validation set. In this experiment, ViT is used for both the oracle backbone and the classifier. The features are 768-dimensional vectors. The classifier is used in the evaluation mode in the experiment.
    % 	\REVISION{\textit{Baseline} indicates ResNet GEM.}
    	}
\end{figure}

==> depd/fig_anal_tsne.tex <==
\begin{figure}[!t]
	\centering
	\subfloat[O: ViT, C: ViT, Loss: CE]{\includegraphics[width=0.24\textwidth]{fig/tsne/tsne_ce}    } \hfill
	\subfloat[O: ViT, C: ViT, Loss: Focal]{\includegraphics[width=0.24\textwidth]{fig/tsne/tsne_focal}    } \hfill
	\subfloat[O: ViT, C: ViT, Loss: TCP]{\includegraphics[width=0.24\textwidth]{fig/tsne/tsne_tcp}    } \hfill
	\subfloat[O: ViT, C: ViT, Loss: SS]{\includegraphics[width=0.24\textwidth]{fig/tsne/tsne_steep}    } \\
	\caption{\label{fig:anal_tsne}
    	Analysis of t-SNE.
    % 	\REVISION{\textit{Baseline} indicates ResNet GEM.}
    	}
\end{figure}

==> depd/tbl_avg_perf.tex <==
\begin{table}[!t]
	\centering
	\caption{\label{tbl:avg_perf}
	    Averaged performance over the regular ImageNet validation set, the stylized ImageNet validation set, and the adversarial ImageNet validation set. The oracle is trained with the cross entropy (CE) loss, the focal loss, and the proposed steep slope (SS) loss on the ImageNet training set. The resulting oracles w.r.t. each loss are evaluated on the three validation sets. The classifier is used in the evaluation mode in the experiment. $d_{KL}$ represents KL divergence, while $c_{B}$ represents Bhattacharyya coefficient.
	}
	\adjustbox{width=1\columnwidth}{
	\begin{tabular}{L{7ex} C{8ex} C{8ex} C{8ex} C{10ex} C{8ex} C{8ex} C{8ex} C{8ex} C{8ex} C{10ex} C{8ex}}
		\toprule
		Loss & C-Acc & $d_{KL}\uparrow$ & $c_{B}\downarrow$ & TPR & TNR & O-Acc & O-Acc\textsubscript{P} & O-Acc\textsubscript{N} & F1 & P & R  \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(lr){9-9} \cmidrule(lr){10-10} \cmidrule(lr){11-11} \cmidrule(lr){12-12}
		& \multicolumn{11}{c}{Oracle: ViT, classifier: ViT} \\
		\cmidrule(lr){2-12}
		CE & 35.74 & 0.5138 & 0.9983 & 99.98 & 0.04 & 35.78 & 35.74 & 0.04 & 0.4382 & 0.3575 & 0.8444 \\
        Focal & 35.74 & 0.5224 & 0.9972 & 99.23 & 1.30 & 36.22 & 35.43 & 0.78 & 0.4374 & 0.3579 & 0.8403 \\
        SS & 35.74 & 1.0875 & 0.9302 & 73.62 & 47.23 & 63.94 & 29.84 & 34.10 & 0.4727 & 0.4430 & 0.5964 \\ \midrule
		& \multicolumn{11}{c}{Oracle: ResNet, classifier: ViT} \\
		\cmidrule(lr){2-12}
		CE & & & & & & & & & & & \\
		Focal & & & & & & & & & & & \\
		SS & & & & & & & & & & & \\
		\bottomrule	
	\end{tabular}}
\end{table}

==> depd/tbl_diff_classifier_oracle.tex <==
\begin{table}[!t]
	\centering
	\caption{\label{tbl:anal_diff}
	    Analysis of the difference of the output features between the classifier backbone and the oracle backbone in terms of $l_{1}$ and $l_{2}$ distances. The common backbone is ViT. The oracle backbone is trained for predicting trustworthiness, while the classifier backbone is pre-trained for classification.
	}
	\adjustbox{width=1\columnwidth}{
	\begin{tabular}{L{7ex} C{14ex} C{14ex} C{14ex} C{14ex}}
		\toprule
		& \multicolumn{2}{c}{Training} & \multicolumn{2}{c}{Validation} \\
		\cmidrule(lr){2-3} \cmidrule(lr){4-5}
		Loss & $l_{1}$ & $l_{2}$ & $l_{1}$ & $l_{2}$ \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5}
		CE & 74.0674$\pm$23.9773 & 3.4074$\pm$1.0967 & 78.4107$\pm$24.9338 & 3.6051$\pm$1.1402 \\
        Focal & 29.0901$\pm$8.5641 & 1.3527$\pm$0.3933 & 30.6497$\pm$8.9262 & 1.4240$\pm$0.4100 \\
        SS & 70.1997$\pm$32.8220 & 3.2129$\pm$1.4973 & 77.3162$\pm$33.4536 & 3.5378$\pm$1.5271 \\
		\bottomrule	
	\end{tabular}}
\end{table}

==> depd/tbl_hindsight_analysis_vit.tex <==
\begin{table}[!t]
	\centering
	\caption{\label{tbl:perf_vit_vit}
	    Hindsight analysis of overall performance using a sliding decision boundary. In this experiment, ViT is used for both the oracle backbone and the classifier. The classifier is used in the evaluation mode in the experiment.
	}
	\adjustbox{width=1\columnwidth}{
	\begin{tabular}{L{7ex} C{8ex} C{8ex} C{8ex} C{10ex} C{8ex} C{8ex} C{8ex} C{8ex} C{8ex} C{10ex} C{8ex} C{8ex} C{8ex} C{8ex} C{8ex}}
		\toprule
		Loss & C-Acc & $d_{KL}$ & $c_{B}$ & TPR & TNR & O-Acc & O-Acc\textsubscript{P} & O-Acc\textsubscript{N} & F1 & P & R \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-16}
		& \multicolumn{15}{c}{Regular validation set} \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-16}
		NLS & & & & & & & & & & & & & & & \\
		Focal & & & & & & & & & & & & & & & \\
		SS & & & & & & & & & & & & & & & \\ \midrule
		& \multicolumn{15}{c}{Stylized validation set} \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-16}
		NLS & & & & & & & & & & & & & & & \\
		Focal & & & & & & & & & & & & & & & \\
		SS & & & & & & & & & & & & & & & \\ \midrule
		& \multicolumn{15}{c}{Adversarial validation set} \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-16}
		NLS & & & & & & & & & & & & & & & \\
		Focal & & & & & & & & & & & & & & & \\
		SS & & & & & & & & & & & & & & & \\
		\bottomrule	
	\end{tabular}}
\end{table}

==> depd/tbl_perf.tex <==
\begin{table}[!t]
	\centering
	\caption{\label{tbl:all_perf}
	    Performance on the ImageNet validation set. The oracles are trained with the ImageNet training samples. The classifier is used in the evaluation mode in the experiment. Acc is the classification accuracy and is helpful to understand the proportion of correct predictions. \textit{SS} stands for the proposed steep slope loss.
	   % For example, Acc=83.90\% implies that 83.90\% of predictions is trustworthy and 16.10\% of predictions is untrustworthy.
	}
	\adjustbox{width=1\columnwidth}{
	\begin{tabular}{C{10ex} L{10ex} C{8ex} C{10ex} C{8ex} C{8ex} C{8ex} C{8ex} C{8ex}}
		\toprule
		\textbf{\textlangle O, C\textrangle} & \textbf{Loss} & \textbf{Acc$\uparrow$} & \textbf{FPR-95\%-TPR$\downarrow$} & \textbf{AUPR-Error$\uparrow$} & \textbf{AUPR-Success$\uparrow$} & \textbf{AUC$\uparrow$} & \textbf{TPR$\uparrow$} & \textbf{TNR$\uparrow$} \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(lr){9-9} 
		\multirow{4}{*}{\textlangle ViT, ViT \textrangle} & CE & 83.90 & 92.83 & \textbf{15.08} & 84.99 & 52.78 & \textbf{100.00} & 0.01 \\
		 & Focal \cite{Lin_ICCV_2017} & 83.90 & 92.68 & 14.69 & 85.46 & 53.47 & 99.06 & 1.61 \\
		 & TCP \cite{Corbiere_NIPS_2019} & 83.90 & 88.07 & 12.86 & 87.80 & 60.45 & 99.72 & 0.00 \\
		 & SS & 83.90 & \textbf{80.89} & 10.31 & \textbf{92.90} & \textbf{73.31} & 88.44 & \textbf{35.64} \\
		\midrule
		\multirow{4}{*}{\textlangle ViT, RSN\textrangle} & CE & 68.72 & 93.10 & 30.93 & 69.10 & 51.26 & \textbf{99.85} & 0.21 \\
		 & Focal \cite{Lin_ICCV_2017} & 68.72 & 94.51 & \textbf{31.47} & 68.57 & 50.40 & 93.25 & 7.33 \\
		 & TCP \cite{Corbiere_NIPS_2019} & 68.72 & 84.16 & 23.15 & 79.85 & 67.09 & 94.33 & 0.00 \\
		 & SS & 68.72 & \textbf{78.09} & 20.94 & \textbf{85.30} & \textbf{74.20} & 67.96 & \textbf{67.80} \\
        \midrule
		\multirow{4}{*}{\textlangle RSN, ViT\textrangle} & CE & 83.90 & 92.58 & 14.59 & 85.57 & 53.78 & \textbf{100.00} & 0.00 \\
		 & Focal \cite{Lin_ICCV_2017} & 83.90 & 94.92 & \textbf{14.87} & 85.26 & 52.49 & \textbf{100.00} & 0.00 \\
		 & TCP \cite{Corbiere_NIPS_2019} & 83.90 & 91.63 & 14.17 & 86.06 & 55.37 & \textbf{100.00} & 0.00 \\
         & SS & 83.90 & \textbf{88.63} & 11.75 & \textbf{89.87} & \textbf{64.11} & 95.41 & \textbf{10.48} \\
% 		RSN & ViT & SS & 83.90 & 89.86 & 11.99 & 89.49 & 62.75 & 67.74 & 48.98 \\
        \midrule
        \multirow{4}{*}{\textlangle RSN, RSN\textrangle} & CE & 68.72 & 94.83 & 29.52 & 70.67 & 52.19 & \textbf{100.00} & 0.00 \\
		 & Focal \cite{Lin_ICCV_2017} & 68.72 & 95.42 & \textbf{30.21} & 69.88 & 51.16 & 99.91 & 0.03 \\
		 & TCP \cite{Corbiere_NIPS_2019} & 68.72 & 88.54 & 24.62 & 77.42 & 62.53 & 99.17 & 0.00 \\
         & SS & 68.72 & \textbf{85.60} & 22.50 & \textbf{81.92} & \textbf{68.08} & 80.44 & \textbf{40.85} \\
		\bottomrule	
	\end{tabular}}
\end{table}

%%% the 1st run results are below
% \begin{table}[!t]
% 	\centering
% 	\caption{\label{tbl:all_perf}
% 	    Performance on the ImageNet validation set. The oracles are trained with the ImageNet training samples. The classifier is used in the evaluation mode in the experiment. Acc is the classification accuracy and is helpful to understand the proportion of correct predictions.
% 	   % For example, Acc=83.90\% implies that 83.90\% of predictions is trustworthy and 16.10\% of predictions is untrustworthy.
% 	}
% 	\adjustbox{width=1\columnwidth}{
% 	\begin{tabular}{C{10ex} L{10ex} C{8ex} C{10ex} C{8ex} C{8ex} C{8ex} C{8ex} C{8ex}}
% 		\toprule
% 		\textbf{\textlangle O, C\textrangle} & \textbf{Loss} & \textbf{Acc$\uparrow$} & \textbf{FPR-95\%-TPR$\downarrow$} & \textbf{AUPR-Error$\uparrow$} & \textbf{AUPR-Success$\uparrow$} & \textbf{AUC$\uparrow$} & \textbf{TPR$\uparrow$} & \textbf{TNR$\uparrow$} \\
% 		\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(lr){9-9} 
% 		\multirow{4}{*}{\textlangle ViT, ViT \textrangle} & CE & 83.90 & 92.83 & \textbf{15.08} & 84.99 & 52.78 & \textbf{100.00} & 0.01 \\
% 		 & Focal \cite{Lin_ICCV_2017} & 83.90 & 92.68 & 14.69 & 85.46 & 53.47 & 99.06 & 1.61 \\
% 		 & TCP \cite{Corbiere_NIPS_2019} & 83.90 & 88.07 & 12.86 & 87.80 & 60.45 & 99.72 & 0.00 \\
% 		 & SS & 83.90 & \textbf{80.89} & 10.31 & \textbf{92.90} & \textbf{73.31} & 88.44 & \textbf{35.64} \\
% 		\midrule
% 		\multirow{4}{*}{\textlangle ViT, RSN\textrangle} & CE & 68.72 & 93.10 & 30.93 & 69.10 & 51.26 & \textbf{99.85} & 0.21 \\
% 		 & Focal \cite{Lin_ICCV_2017} & 68.72 & 94.51 & \textbf{31.47} & 68.57 & 50.40 & 93.25 & 7.33 \\
% 		 & TCP \cite{Corbiere_NIPS_2019} & 68.72 & 84.16 & 23.15 & 79.85 & 67.09 & 94.33 & 0.00 \\
% 		 & SS & 68.72 & \textbf{78.09} & 20.94 & \textbf{85.30} & \textbf{74.20} & 67.96 & \textbf{67.80} \\
%         \midrule
% 		\multirow{4}{*}{\textlangle RSN, ViT\textrangle} & CE & 83.90 & 92.58 & 14.59 & 85.57 & 53.78 & \textbf{100.00} & 0.00 \\
% 		 & Focal \cite{Lin_ICCV_2017} & 83.90 & 94.92 & \textbf{14.87} & 85.26 & 52.49 & \textbf{100.00} & 0.00 \\
% 		 & TCP \cite{Corbiere_NIPS_2019} & 83.90 & 91.63 & 14.17 & 86.06 & 55.37 & \textbf{100.00} & 0.00 \\
%          & SS & 83.90 & \textbf{88.63} & 11.75 & \textbf{89.87} & \textbf{64.11} & 95.41 & \textbf{10.48} \\
% % 		RSN & ViT & SS & 83.90 & 89.86 & 11.99 & 89.49 & 62.75 & 67.74 & 48.98 \\
%         \midrule
%         \multirow{4}{*}{\textlangle RSN, RSN\textrangle} & CE & 68.72 & 94.83 & 29.52 & 70.67 & 52.19 & \textbf{100.00} & 0.00 \\
% 		 & Focal \cite{Lin_ICCV_2017} & 68.72 & 95.42 & \textbf{30.21} & 69.88 & 51.16 & 99.91 & 0.03 \\
% 		 & TCP \cite{Corbiere_NIPS_2019} & 68.72 & 88.54 & 24.62 & 77.42 & 62.53 & 99.17 & 0.00 \\
%          & SS & 68.72 & \textbf{85.60} & 22.50 & \textbf{81.92} & \textbf{68.08} & 80.44 & \textbf{40.85} \\
% 		\bottomrule	
% 	\end{tabular}}
% \end{table}

==> depd/tbl_perf_avg.tex <==
\begin{table}[!t]
	\centering
	\caption{\label{tbl:all_perf}
	    Performance on the ImageNet validation set. The averaged scores are computed over three runs. The oracles are trained with the ImageNet training samples. The classifier is used in the evaluation mode in the experiment. Acc is the classification accuracy (\%) and is helpful to understand the proportion of correct predictions. \textit{SS} stands for the proposed steep slope loss.
	   % For example, Acc=83.90\% implies that 83.90\% of predictions is trustworthy and 16.10\% of predictions is untrustworthy.
	}
	\adjustbox{width=1\columnwidth}{
	\begin{tabular}{C{10ex} L{9ex} C{8ex} C{10ex} C{8ex} C{8ex} C{8ex} C{8ex} C{8ex}}
		\toprule
		\textbf{\textlangle O, C\textrangle} & \textbf{Loss} & \textbf{Acc$\uparrow$} & \textbf{FPR-95\%-TPR$\downarrow$} & \textbf{AUPR-Error$\uparrow$} & \textbf{AUPR-Success$\uparrow$} & \textbf{AUC$\uparrow$} & \textbf{TPR$\uparrow$} & \textbf{TNR$\uparrow$} \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(lr){9-9} 
		\multirow{4}{*}{\textlangle ViT, ViT \textrangle} & CE & 83.90 & 93.01 & \textbf{15.80} & 84.25 & 51.62 & \textbf{99.99} & 0.02 \\
		 & Focal \cite{Lin_ICCV_2017} & 83.90 & 93.37 & 15.31 & 84.76 & 52.38 & 99.15 & 1.35 \\
		 & TCP \cite{Corbiere_NIPS_2019} & 83.90 & 88.38 & 12.96 & 87.63 & 60.14 & 99.73 & 0.00 \\
		 & SS & 83.90 & \textbf{80.48} & 10.26 & \textbf{93.01} & \textbf{73.68} & 87.52 & \textbf{38.27} \\
		\midrule
		\multirow{4}{*}{\textlangle ViT, RSN\textrangle} & CE & 68.72 & 93.43 & 30.90 & 69.13 & 51.24 & \textbf{99.90} & 0.20 \\
		 & Focal \cite{Lin_ICCV_2017} & 68.72 & 93.94 & \textbf{30.97} & 69.07 & 51.26 & 93.66 & 7.71 \\
		 & TCP \cite{Corbiere_NIPS_2019} & 68.72 & 83.55 & 23.56 & 79.04 & 66.23 & 94.25 & 0.00 \\
		 & SS & 68.72 & \textbf{77.89} & 20.91 & \textbf{85.39} & \textbf{74.31} & 68.32 & \textbf{67.53} \\
        \midrule
		\multirow{4}{*}{\textlangle RSN, ViT\textrangle} & CE & 83.90 & 93.29 & 14.74 & 85.40 & 53.43 & \textbf{100.00} & 0.00 \\
		 & Focal \cite{Lin_ICCV_2017} & 83.90 & 94.60 & \textbf{14.98} & 85.13 & 52.37 & \textbf{100.00} & 0.00 \\
		 & TCP \cite{Corbiere_NIPS_2019} & 83.90 & 91.93 & 14.12 & 86.12 & 55.55 & \textbf{100.00} & 0.00 \\
         & SS & 83.90 & \textbf{88.70} & 11.69 & \textbf{90.01} & \textbf{64.34} & 96.20 & \textbf{9.00} \\
% 		RSN & ViT & SS & 83.90 & 89.86 & 11.99 & 89.49 & 62.75 & 67.74 & 48.98 \\
        \midrule
        \multirow{4}{*}{\textlangle RSN, RSN\textrangle} & CE & 68.72 & 94.84 & 29.41 & 70.79 & 52.36 & \textbf{100.00} & 0.00 \\
		 & Focal \cite{Lin_ICCV_2017} & 68.72 & 95.16 & \textbf{29.92} & 70.23 & 51.43 & 99.86 & 0.08 \\
		 & TCP \cite{Corbiere_NIPS_2019} & 68.72 & 88.81 & 24.46 & 77.79 & 62.73 & 99.23 & 0.00 \\
         & SS & 68.72 & \textbf{86.21} & 22.53 & \textbf{81.88} & \textbf{67.92} & 79.20 & \textbf{42.09} \\
		\bottomrule	
	\end{tabular}}
\end{table}

==> depd/tbl_perf_featinput_vit_vit.tex <==
\begin{table}[!t]
	\centering
	\caption{\label{tbl:anal_featinput}
	    Analysis of taking the features of the classifier as input to the oracle on the ImageNet validation set. In this experiment, ViT is used for both the oracle backbone and the classifier. The features are 768-dimensional vectors. The classifier is used in the evaluation mode in the experiment.
	}
	\adjustbox{width=1\columnwidth}{
	\begin{tabular}{L{7ex} C{8ex} C{8ex} C{8ex} C{10ex} C{8ex} C{8ex} C{8ex} C{8ex} C{8ex} C{8ex} C{8ex}}
		\toprule
		Loss & C-Acc & $d_{KL}\uparrow$ & $c_{B}\downarrow$ & TPR & TNR & O-Acc & O-Acc\textsubscript{P} & O-Acc\textsubscript{N} & F1 & P & R \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(lr){9-9} \cmidrule(lr){10-10} \cmidrule(lr){11-11} \cmidrule(lr){12-12}
		CE & 83.90 & 0.5139 & 0.9983 & 100.00 & 0.01 & 83.90 & 83.90 & 0.00 & 0.9125 & 0.8390& 1.0000 \\
        Focal & 83.90& 0.5182 & 0.9977 & 99.06 & 1.61 & 83.36& 83.10 & 0.26 & 0.9090 & 0.8399& 0.9906 \\
        SS & 83.90 & 1.2088 & 0.9155& 91.28 & 28.02 & 81.09 & 76.58 & 4.51 & 0.8902 & 0.8686 & 0.9128 \\ 
		\bottomrule	
	\end{tabular}}
\end{table}

==> depd/tbl_perf_rsn_vit.tex <==
\begin{table}[!t]
	\centering
	\caption{\label{tbl:perf_rsn_vit}
	    Performances on the regular ImageNet validation set, the stylized ImageNet validation set, and the adversarial ImageNet validation set. In this experiment, ResNet-50 is used for the oracle backbone while ViT is used for the classifier. The classifier is used in the evaluation mode in the experiment.
	}
	\adjustbox{width=1\columnwidth}{
	\begin{tabular}{L{8ex} C{8ex} C{8ex} C{8ex} C{10ex} C{8ex} C{8ex} C{8ex}}
		\toprule
		Loss & Acc$\uparrow$ & FPR-95\%-TPR$\downarrow$ & AURP-Error$\uparrow$ & AURP-Success$\uparrow$ & AUC$\uparrow$ & TPR$\uparrow$ & TNR$\uparrow$ \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8}
		& \multicolumn{7}{c}{Regular validation set} \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-8}
		CE & 83.90 & 92.58 & 14.59 & 85.57 & 53.78 & 100.00 & 0.00 \\
		Focal & 83.90 & 94.92 & 14.87 & 85.26 & 52.49 & 100.00 & 0.00 \\
		TCP & 83.90 & 91.63 & 14.17 & 86.06 & 55.37 & 100.00 & 0.00 \\
% 		SS & 83.90 & 89.86 & 11.99 & 89.49 & 62.75 & 67.74 & 48.98 \\
		SS & 83.90 & 88.63 & 11.75 & 89.87 & 64.11 & 95.41 & 10.48 \\
% 		& 83.90 & 88.63 & 11.75 & 89.87 & 64.11 & 95.41 & 10.48 \\
%         & 83.90 & 88.72 & 11.76 & 89.85 & 64.01 & 91.10 & 18.51 \\
% 		& 83.90 & 88.25 & 11.54 & 90.24 & 65.23 & 88.23 & 24.25 \\ rsn152
		\midrule
		& \multicolumn{7}{c}{Stylized validation set} \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-8}
		CE & 15.94 & 86.54 & 79.32 & 22.00 & 61.74 & 100.00 & 0.00 \\
		Focal & 15.94 & 95.04 & 85.18 & 14.94 & 48.20 & 100.00 & 0.00 \\
		TCP & 15.94 & 90.82 & 80.69 & 19.96 & 58.34 & 100.00 & 0.00 \\
		SS & 15.94 & 93.80 & 82.10 & 18.19 & 54.18 & 56.94 & 48.88 \\
% 		& 15.94 & 94.27 & 83.09 & 16.97 & 52.35 & 92.13 & 9.03 \\ 52
% 		& 15.94 & 95.76 & 84.28 & 15.74 & 49.02 & 93.83 & 5.52 \\ a62
        \midrule
		& \multicolumn{7}{c}{Adversarial validation set} \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-8}
        CE & & & & & & &  \\
        Focal & & & & & & &  \\
        TCP & & & & & & & \\
        SS & & & & & & &  \\
		\bottomrule	
	\end{tabular}}
\end{table}

==> depd/tbl_perf_vit_vit_old.tex <==
\begin{table}[!t]
	\centering
	\caption{\label{tbl:perf_vit_vit}
	    Performances on the regular ImageNet validation set, the stylized ImageNet validation set, and the adversarial ImageNet validation set. In this experiment, ViT is used for both the oracle backbone and the classifier. The oracle is trained with the CE loss, the focal loss, and the proposed steep slope loss on the ImageNet training set. The resulting oracles w.r.t. each loss are evaluated on the three validation sets. The classifier is used in the evaluation mode in the experiment.
	}
	\adjustbox{width=1\columnwidth}{
	\begin{tabular}{L{7ex} C{8ex} C{8ex} C{8ex} C{10ex} C{8ex} C{8ex} C{8ex} C{8ex} C{8ex} C{8ex} C{8ex}}
		\toprule
		Loss & C-Acc & $d_{KL}\uparrow$ & $c_{B}\downarrow$ & TPR & TNR & O-Acc & O-Acc\textsubscript{P} & O-Acc\textsubscript{N} & F1 & P & R \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(lr){9-9} \cmidrule(lr){10-10} \cmidrule(lr){11-11} \cmidrule(lr){12-12}
		& \multicolumn{11}{c}{Regular validation set} \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-12}
		CE & 83.90 & 0.5139 & 0.9983 & 100.00 & 0.01 & 83.90 & 83.90 & 0.00 & 0.9125 & 0.8390& 1.0000 \\
        Focal & 83.90& 0.5182 & 0.9977 & 99.06 & 1.61 & 83.36& 83.10 & 0.26 & 0.9090 & 0.8399& 0.9906 \\
        SS & 83.90 & 1.2088 & 0.9155& 91.28 & 28.02 & 81.09 & 76.58 & 4.51 & 0.8902 & 0.8686 & 0.9128 \\ 
		\midrule
		& \multicolumn{11}{c}{Stylized validation set} \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-12}
		CE & 15.93 & 0.5017 & 0.9998 & 99.99 & 0.02 & 15.95 & 15.93 & 0.02 & 0.2749 & 0.1594 & 0.9999 \\
        Focal & 15.93 & 0.5202 & 0.9975 & 99.71 & 00.25& 16.09 & 15.89 & 0.20 & 0.2747 & 0.1593 & 0.9971 \\
        SS & 15.93 & 1.1616 & 0.9225 & 39.17 & 87.41 & 79.72 & 6.24 & 73.48 & 0.3810 & 0.3709 & 0.3917 \\ \midrule
		& \multicolumn{11}{c}{Adversarial validation set} \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-12}
		CE& 7.4040 & 0.5260 & 0.9968 & 99.95 & 0.11 & 7.50 & 7.40 & 0.10 & 0.1274 & 0.0741 & 0.5333 \\
        Focal & 7.4040 & 0.5290 & 0.9964 & 98.92 & 2.05 & 9.22 & 7.32 & 1.90 & 0.1285 & 0.0747& 0.5333 \\
        SS& 7.4040 & 0.8922 & 0.9527 & 90.42 & 26.26 & 31.02 & 6.70 & 24.32 & 0.1470 & 0.0896 & 0.4848 \\
		\bottomrule	
	\end{tabular}}
\end{table}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> rebuttal/discussion.tex <==
Just recall that somehow I thought as long as we convinced the reviewers that the other works are not as good as the TCP design, [2] is not relevant. But in fact, we did not rebut this one "Recent (parallel) work [2] has benchmarked these methods on large-scale datasets which indicates these scale well to larger datasets.", which may affect our claim on large-scale.

Yan Luo  10:52 PM
ref 2 is ood detection，in my view，2 is out of context and irrelevant. Lets say if relevant，this implies that all trustworthiness works should take ood models as baseline
10:53
I guess the reviewer is the author of 2 and feel the prob is super useful so recommend to us by showing that prob has many applications

Catherine Zhao  10:55 PM
could be
10:56
yeah, hard choice, we cannot say negative words about it (like not as good as us), so maybe leaving it is fine
10:56
though it may give the impression that we skipped this one [2]

Yan Luo  10:59 PM
We bury a bullet for this point by leaving a sentence which is not the goal of OOD detection. We are waiting for the reviewer rasing that question

Catherine Zhao  11:03 PM
ok, so the point is that [2] targets OOD, which should not be the goal for all trustworthy papers?
11:03
we did not convey any points though as we did not mention [2]
11:04
the sentence "However, we would like to point out that trustworthiness informs whether one can safely use the predictions yielded by AI for making decisions, which is not the goal of out-of-distribution detection." to me simply means that OOD has other goals and is different from trustworthy problems.

Yan Luo  11:25 PM
Let us look a an example，we train a model with real world cat image，and expect the model can detect cartoon cat as well. it could fail to detect a cartoon image. So ood image is a factor affecting trustworthiness，but that is not all the reasons. There are many facotrs affecting TW，like the deep learming models are not perfect to classify in diatribution images，and real world cat is semantically complicated to be perfectly classified

==> sec/misc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section 1.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    % \answerTODO{}
    \answerYes{}
  \item Did you describe the limitations of your work?
    % \answerTODO{}
    \answerYes{Please see the discussion in the ablation study in Section \ref{sec:exp}}
  \item Did you discuss any potential negative societal impacts of your work?
    % \answerTODO{}
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    % \answerTODO{}
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    % \answerTODO{}
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    % \answerTODO{}
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    % \answerTODO{}
    \answerYes{Please refer to the abstract, the experimental set-up in Section \ref{sec:exp}, and Section \ref{sec:implementation} in the appendix.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    % \answerTODO{}
    \answerYes{Please refer to the experimental set-up and the ablation study in Section \ref{sec:exp}, and Section \ref{sec:implementation} in the appendix.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    % \answerTODO{}
    \answerYes{Please refer to \tabref{tbl:all_perf}, \tabref{tbl:all_perf_w_std}, and Section \ref{sec:implementation} in the appendix.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    % \answerTODO{}
    \answerYes{Please refer to Section \ref{sec:implementation} in the appendix.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Please refer to Section \ref{sec:exp} and Section \ref{sec:implementation} in the appendix.}
  \item Did you mention the license of the assets?
    % \answerTODO{}
    \answerYes{Please refer to Section \ref{sec:license} in the appendix.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Please refer to the abstract and Section \ref{sec:license} in the appendix.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content? 
    \answerYes{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \appendix

% \section{Appendix}

% Optionally include extra information (complete proofs, additional experiments and plots) in the appendix.
% This section will often be part of the supplemental material.
